BagPipe: Accelerating Deep Recommendation Model Training

Deep learning based recommendation models (DLRM) are widely used in several business critical applications. Training such recommendation models efficiently is challenging because they contain billions of embedding-based parameters, leading to significant overheads from embedding access. By profiling existing systems for DLRM training, we observe that around 75\% of the iteration time is spent on embedding access and model synchronization. Our key insight in this paper is that embedding access has a specific structure which can be used to accelerate training. We observe that embedding accesses are heavily skewed, with around 1\% of embeddings representing more than 92\% of total accesses. Further, we observe that during offline training we can lookahead at future batches to determine exactly which embeddings will be needed at what iteration in the future. Based on these insights, we develop Bagpipe, a system for training deep recommendation models that uses caching and prefetching to overlap remote embedding accesses with the computation. We design an Oracle Cacher, a new component that uses a lookahead algorithm to generate optimal cache update decisions while providing strong consistency guarantees against staleness. We also design a logically replicated, physically partitioned cache and show that our design can reduce synchronization overheads in a distributed setting. Finally, we propose a disaggregated system architecture and show that our design can enable low-overhead fault tolerance. Our experiments using three datasets and four models show that Bagpipe provides a speed up of up to 5.6x compared to state of the art baselines, while providing the same convergence and reproducibility guarantees as synchronous training.

==> bagpipe_old.tex <==
\section{\system{} Design}



% The Trainers are synchronized using Allreduce primitives.

\subsection{Design Overview}
%To enable large scale recommendation model training,
\system introduces three major design contributions:

%\system is a system designed for efficient large scale recommendation training. For efficient large scale training  
\begin{myitemize}

\item First, we design a new embedding caching mechanism that can exploit the skew in access patterns while handling changes in popularity and long tail accesses. We introduce a dynamic \emph{oracular} cache that is designed to \emph{lookahead} at future training batches to determine cache insertions and evictions. We discuss how this insight can be used in a single machine in Section~\ref{sec:caching_in_bagpipe} and extend our design to a distributed setup in Section~\ref{sec:dist_cache}.
%Detailed design and analysis of our caching mechanism can be found 

\item Second, in contrast to existing training setups (Figure~\ref{fig:existing_training_setup}) \system{} uses a dis-aggregated architecture which can independently scale embedding table partitions and trainers depending on the properties of recommendation model being trained. Figure~\ref{fig:bagpipe_training_setup} provides an overview of \system{} system design and we show how our design can also improve fault tolerance in Section~\ref{sec:system_design}.
%and also .
 
\item Third, \system{} is designed to pipeline or overlap communication and cache management with the compute in model training.
We present strategies to maximize the overlap and increase resource utilization in Section~\ref{sec:bagpipe_overlap}.
%and thereby m from the critical path.
\end{myitemize}




% required
% \begin{figure}[t] 
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/all_to_all.pdf}
%     \vspace{-0.1in}
%     \caption{\small{\textbf{All2All op} }}
%     \label{fig:all2all}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/dependency_graph_dlrm.pdf}
%     \vspace{-0.1in}
%     \caption{\small{\textbf{DLRM Dependency Graph} }}
%     \label{fig:dlrm_dependency_graph}
% \end{figure}tab:
  \begin{figure*}[t]
    \includegraphics[width=0.9\linewidth]{images/oracle_cacher_schematic.pdf}
    \centering
    \vspace{-0.12in}
    \caption{\small{\textbf{Lookahead Algorithm}: The above figure shows an illustration at different batch steps how lookahead algorithm functions. In the above example the lookahead value is 2 and the batch size is also 2.}}
    \label{fig:oracle_cacher_example}
    \vspace{-17pt}
    \end{figure*}
    
    
 
\subsection{Caching in \system}
\label{sec:caching_in_bagpipe}
%As discussed in Section~\ref{sec:existing_method} and shown in Figure~\ref{fig:hit_rate_batch} static caching is not able to provide promised speedups. 
%Methods which have been proposed to gain speedup from static caching like FAE~\cite{adnan2021high} often have accuracy implications and require significant amount of pre-processing.
We design a dynamic cache that can add and evict elements dynamically by analyzing batches that will be trained in the future. For this purpose we introduce the idea of \emph{Lookahead}, where we can make a decision of what entries need to be cached based on future access patterns. Specifically we denote \lkval, or lookahead value, as the number of batches ahead of the current batch we are going to look at. For example, if the current batch is $x$, we consider data accesses in batches from $x$ to $x$+\lkval, to determine which elements in batch $x$ should be cached.
Given this approach we next discuss how a cache can be maintained in a single GPU setting based. Then we discuss design strategies to extend this to a distributed setting.
%Next we introduce various components which enable caching in \system. 





% To reduce the overhead of synchronization we only synchronize the elements which have been updated in previous rounds.

% \noindent\textbf{Synchronizing Caches.}\saurabh{Replicated Caches need to be synchronized. We perform two additional optimization. First of all instead of synchronizing the whole cache we only synchronize the gradients of the elements which have been updated in the current iteration. Next we perform an additional optimization in which we first only sync the elements which will be required in the next iteration, and we schedule rest of the elements to be synchronized in the background. Thus only a very small portion of the elements are synchronized on the critical path. This optimization enables us to overlap a large portion of cache synchronization with compute. We evaluate the effect of this optimization in Section~\ref{sec:}}

% One of the most important decisions when performing caching is deciding what to cache. 

\label{sec:lookahead_routine}
\paragraph{Deciding what to cache and for how long.} To decide what to cache \system relies on one key insight: \emph{in offline batch training future batches and their contents are predictable}, \ie we can look beyond current batch and find out which embeddings will be accessed by future batches. This insight enables \system to look-ahead beyond the current batch and create a perfect or an \emph{oracular} cache~\cite{belady1966study}.
% Cite https://ieeexplore.ieee.org/document/5388441

For deciding what to cache and what to evict we develop a low overhead (benchmark in Section~\ref{sec:oracle_cacher_benchmark}) lookahead algorithm (Algorithm~\ref{alg:lookaheadalg}) that also ensures consistent access to embeddings. We denote the  \emph{lookahead value} (\lkval), as the number of batches ahead of the current batch we are going to analyze to determine what to cache. The lookahead algorithm takes three inputs: the current batch, future batches  (as many required for lookahead) and current state of the dynamic cache. 
%For example, if the lookahead routine is processing batch number $x$ and lookahead value is set to $y$, the lookahead routine will need the current batch $x$ and next $y$ batches of training data. 
The lookahead algorithm outputs two pieces of information. %\shivaram{make it two pieces and say everything is just ttl?}
First, for the current batch, it generates the list of embeddings which will not be found in the cache on the trainer GPUs. This allows us to \emph{prefetch} these embeddings and move those elements into the cache, before the current training batch is used for training. Prefetching allows \system{} to hide the data access latency for the long tail of embeddings that are not frequently accessed. 
% early
%This guarantees that when batch is loaded for training it will find all the necessary embeddings in the dynamic local cache. 
% within the future batches
Second, the lookahead algorithm determines \emph{which embeddings \textbf{from the current batch} will be used in future batches} and the last iteration they will be accessed in. Any embeddings from the current batch that will be used by any of the future batches within the \emph{lookahead} window will be marked for caching, so they can be accessed from the GPU memory in future. The last iteration an embedding is used within the \emph{lookahead} range serves as time-to-live (TTL) for the embedding in the cache.
% Third, the lookahead algorithm determines the time-to-live (TTL) for each element in the cache. We next describe the details of our lookahead algorithm.

 
\paragraph{Lookahead Algorithm.}
Our lookahead algorithm (Algorithm~\ref{alg:lookaheadalg}) takes in the preset lookahead value (\lkval) as an argument and dynamically keeps a window of batches of that size. The window is maintained as a queue, where the next batch to be processed is in the front of the queue. As shown in Line 5-12, when the window size is smaller than the look-ahead value (at the beginning of the training or after a batch is processed), the algorithm extends the window by reading new batches from the data loader. Meanwhile, it also keeps the last occurrence of each embedding in this window. After ensuring that the window size is equal to \lkval (or there are no more batches to process), the algorithm starts to process the first batch in the window, as shown in Line 15-27. For each embedding in the batch, we add a TTL update to denote the latest occurrence of this embedding, and then add a pre-fetch request if this embedding is not in cache.
% Suppose the current batch number is $x$.

%In Line 25, we also safely erase embedding $e$ from $LatestTracker$ if $e$ is not in the cache to ensure that the memory complexity is linear to the number of embeddings that appear in the window. 
%This is an update to the cache status that is maintained locally.

% Using an default dictionary in Python for both $InCache$ and $LatestTracker$, we only need a constant number of work for each embedding in each batch. Therefore, we have an implementation of time complexity $O(m)$ for each batch, where $m$ is the number of embeddings in each batch. Thus the algorithm has a very low overhead on the training process.

We next take a look at an example of the lookahead algorithm in action in Figure~\ref{fig:oracle_cacher_example}. We use a lookahead value (\lkval) as 2 and show how a window of batches are processed by the lookahead algorithm.
%taken by the oracle cacher  and producing cache update requests. 
%The local embedding cache in Figure~\ref{fig:oracle_cacher_example} keeps track of what is in the $InCache$ variable in the algorithm.

\begin{myitemize}
  \item \textbf{Batch 1} Embedding 3 and 9 are in the batch. For both embedding 3 and 9, we will launch prefetches. However, for embedding 3, we see that it is accessed again, and last occurrence in the window is at Batch 2, so we decide to cache it with the TTL set to 2. 
  \item \textbf{Batch 2} For embedding 3, we see that it is in the cache but last occurrence in the window is in now Batch 3. So we will send a TTL update for 3. We will not launch a prefetch for 3 because 3 is already in the cache, while we will prefetch 4 since it is not in the cache. 
  
  \item \textbf{Batch 3} For embedding 3, we do not see any future occurrence in the window, so we will not send any TTL updates. For embedding 6, we decide to cache it with a TTL of 4 because it will be used in Batch 4. Embedding 3 will be deleted from the cache after this batch.
  
  \item \textbf{Batch 4} For this iteration, we will prefetch 1 since it is not in the cache. We do not send any TTL updates for 6 as it is absent in future batches. It will be deleted from the cache after this batch.
  \end{myitemize}



\noindent\textbf{Consistency Guarantee.}
%\shivaram{old invariant para from above is commented out here.}
%The above steps provide an invariant that is crucial for ensuring consistent access. For an embedding $e$, suppose the last iteration it appears in (including the current one) is $x$. $InCache$ has $e$ if and only if it had previous occured at iteration $y$ such that $y - x < \text{\lkval} $. We maintain this invariant in Line 21 and 24. This guarantees that when the iteration $y$ starts, the trainer will only pre-fetch $e$ when $e$ did not appear in any batch in the range of [y - \lkval, y). This ensures that there are no conflicts between embeddings in cache and those that are being fetched.
% To guarantee same result as synchronous training we need to make sure that the latest updated value of the embedding is read for next training iteration. 
Our key consistency goal is to avoid staleness and ensure that workers do not pre-fetch an embedding from the embedding servers while it has updates that have not yet been written back. %we need to make sure that the latest updated value of the embedding is always used as in synchronous training. 
Despite pre-fetching embeddings out of order, 
% \shivaram{We need to read the latest value. Explain that in case of prefetch it is not obvious.}
 our formulation of what to cache and when to prefetch as described by Algorithm~\ref{alg:lookaheadalg}, provides a subtle but an extremely important guarantee that allows us to maintain consistency and match the execution of synchronous training. 
 % minimize communication overheads while
 
%  We reemphasize on how 
%  The invariant derived in Algorithm~\ref{alg:lookaheadalg} enables consistency despite out of order prefetching. 
%  The invariant derived in lookahead algorithm enables us to do this. 
% will  when the batch is processed going to 
 When the lookahead algorithm is processing batch number $x$, an embedding used by the batch will either be available in the cache with the most recent value or no preceding batch in the lookahead range (any batch number in [$x - \text{\lkval}, x)$) would have updated that specific embedding. In other words, if an embedding was needed by a batch in batch number in range $[x-\text{\lkval}, x)$ it will be in the cache; if an embedding is not in the cache it means no batch in range of $[x-\text{\lkval}, x)$ has updated it. Therefore, as long as the prefetch request is issued after updates from training batch number $x - \text{\lkval}$ have been written back, we can safely prefetch embeddings without being concerned about staleness. This condition guarantees that despite fetching embeddings out of order we will still see the same results as synchronous training. 
%  will need an embedding
% value number of 
%  will be used in the next

% To emphasize this again but in a slightly different manner

% for a given duration
% reason about

% providing the same guarantees
% cache to hold frequently used embeddings in the GPU memory

\subsection{Distributed Caching}
\label{sec:dist_cache}
Next we look at how to extend our cache to a distributed setup. We consider a setup where we have $p$ machines with each machine having a fixed-size cache. We compare two approaches: exclusive and replicated caches, and analyze them in terms of communication incurred and state maintenance. 

\noindent\textbf{Exclusive vs. Replicated Caches.}
Given a cluster of $p$ machines, at a high level we have three design choices: replicated, exclusive or a hybrid cache (mix of both replicated and exclusive). In an exclusive cache, only one machine in the cluster can hold an embedding in cache and any other machine which needs to access the embedding performs a peer to peer (P2P) access to fetch the embedding and then writes back the gradient at the end of a batch. In the case of a replicated cache all the elements in the cache are present on all the machines and after training a batch we synchronize elements (e.g., using AllReduce) that were updated in this batch. Finally a hybrid cache can be designed to have some portion of the cache be replicated while the remaining entries are exclusive. 

% accessed 
% Since we want to to minimize the overhead in our caching logic we do not aim trainers we reduce the training time 
% cache setup When building distributed caches we can have three choices. 

% \shivaram{Flow: Let us assume we do pre-fetching and routing at random. (otherwise routing overhead is too high. Can we prove?). Given that we have three choices.
% 1. We can use exclusive caches. so one machine owns an element and we do p2p access to fetch.
% 2. we can use replicated caches. so all machines can read locally. need to sync updated embeddings after end of iteration
% 3. we can use a combination of the two. Some parts are replicated (thresholding).
% We run a simulation comparing these three approaches in terms of amount of comm on critical path. We quantify it in terms of bytes read/written by bottleneck worker.
% Observations: }
\noindent\textbf{Communication.} 
The amount of communication incurred in a replicated vs. exclusive cache depends on the data access patterns on each machine. In the case where there is no significant overlap between embeddings being accessed by different machines an exclusive cache is expected to perform better. This is because the replicated cache would incur additional overheads in synchronizing embeddings that are only updated on a single machine. On the other hand when there is a large overlap between machines a replicated cache is expected to perform better. In the extreme where all machines update the same set of embeddings (similar to a data-parallel DNN), a replicated cache can use efficient collective primitives to perform the synchronization.

To evaluate the design choices we simulated the amount of synchronization that will be required for three datasets (Table~\ref{tab:datasets}). Further, based on the amount of communication derived from simulation, we performed the same amount of communication on a real cluster using the best available communication primitives and calculated the total time required for communication. In our simulation, we dispatched examples to machines at random in order to minimize overhead for our example dispatcher.
%as any cache aware routing will require extra control logic and possibly limit scalability.
We observed that for training one epoch of the Kaggle Criteo dataset with a batch size of 16,384, the total synchronization time is similar for both Exclusive and Replicated cache (around 25 seconds). In terms of communication, for exclusive caches each node on average reads ~12K embeddings and writes back around ~12K embeddings (total ~24K), while for replicated caches the nodes on average synchronize around 22K embeddings. We see similar trends for the other two datasets as well.
%The reason is that the large size of embedding table makes it hard to find efficient algorithms to find a partition that significantly saves communication (is this ok?) (ziyi's point)

% \ziyi {When partitioning the examples and the cache contents (in case of exclusive cache), we will assume uniformly random partition across all the workers. The reason is that the large size of embedding table makes it hard to find efficient algorithms to find a partition that significantly saves communication (is this ok?).  There are two representative choices for the cache. 
% \begin{itemize}
%   \item The first one is an exclusive cache, where the cache content is partitioned into different machines, i.e. each embedding in the cache only exists in one of the machines. Therefore, before the computation of each training iterations, each worker has to fetch the needed non-local embeddings from other workers, and after the computation, each worker will send the gradient updates back to other workers.
%   \item The other one is a replicated cache, where the cache content is replicated across all the machines. Before the computation of each training iterations, no fetch is required because every embedding is local. After the computation, each worker will need to synchronize the gradients and update all the embeddings in each worker.
% \end{itemize}
% Besides those two representaitive cases, we could as well do a hybrid cache where the hot embeddings are replicated across each machine while the others are partitioned acroos different machines. }
\noindent\textbf{State.} Given that synchronization costs are similar, we next compare the two approaches in terms of the state that needs to be maintained. We observe that if we use a replicated cache %it will require additional control logic to determine where each trainer should send a request to fetch the embeddings, \ie,  focus on other properties which can make one design choice better than the other.
we will not need to maintain any extra state for determining which machine owns which embedding. Further, with a replicated cache each trainer will have the same state thus making fault tolerance and recovery significantly easier (Details in Section~\ref{sec:ft}). 
On the other hand, the exclusive cache can hold more unique embeddings given a fixed memory budget.  However, from our experiments we observe that 
even for large \lkval values we only need around a gigabyte of GPU memory for all the embeddings that need to be cached (Figure~\ref{fig:effect_of_lookahead_cache_size}). In practice it is feasible to store 1GB on each machine as With a local batch size of 2048 only 1.8GB of memory out of 16 GB on a V100 is used by the DLRM model, leaving almost 14 GB free.  Finally, the hybrid cache suffers from the issues faced by both replicated and exclusive cache; the state on each trainer will be different making fault tolerance expensive while also needing additional state for determining which machines owns which embedding.
Based on the above exploration, we use a \emph{replicated} dynamic cache in \system{}.

% than a non-replicated cache.
% \shivaram{what did we do in the simulation. give some concrete numbers about comm overhead.}
% \shivaram{Nice properties that replicated cache has 
% 1. no need to tag which machine to read from
% 2. fault recovery of the oracle cacher. fault recovery of trainer.
% downside is
% 1. needs more memory}
%There are two main concerns that we need to consider when distributing   



% A gigabyte of memory is easily available on modern GPUs even for the most compute intensive recommendation models. 

% Secondly, a non-replicated cache will require additional control logic to provide load balancing and synchronization, which can make our training batch dispatch quite slow. Therefore, we chose to use a replicated cache. The main overhead in using a replicated cache is that its contents have to be synchronized at the end of every training iteration. In Section~\ref{sec:bagpipe_overlap} we discuss how we are able to move a significant portion of synchronization out of the critical path and overlap it with forward and backward pass.
 


%\paragraph{Dynamic and Replicated Cache.} 

% \paragraph{Guaranteeing Consistency.}
% To guarantee same result as synchronous training we need to make sure that the updated value of the embedding is read for next training iteration. Despite pre-fetching embeddings out of order, 
% % \shivaram{We need to read the latest value. Explain that in case of prefetch it is not obvious.}
%  our formulation of what to cache and when to prefetch, provides a subtle but an extremely important guarantee that allows us to minimize communication overheads while matching the execution of synchronous training.
%  The key consistency goal in our design is to ensure that workers do not pre-fetch an embedding from the embedding servers while it has updates in cache that have not been written back.
%  To achieve this goal, we derive an invariant that the lookahead algorithm maintains. When lookahead algorithm is processing batch number $x$, either an embedding needed by the batch with its most updated value will be available in the cache when the batch is processed or no preceding batch in the lookahead range (any batch number in [$x - \text{\lkval}, x)$) is going to update that specific embedding. To emphasize this again but in a slightly different manner, if an embedding was needed by a batch in batch number in range $[x-\text{\lkval}, x)$ it will be in the cache; if it is not in the cache it means no batch in range of $[x-\text{\lkval}, x)$ has updated it. Therefore, as long as the prefetch request is issued after updates from training batch number $x - \text{\lkval}$ have been written back, we can safely prefetch embeddings without being concerned about staleness. This specific condition guarantees that despite fetching embeddings out of order we will still see the same results as synchronous training. 
 
 %This is very similar to out-of-order execution performed in modern microprocessors. 
% \subsection{\system Motivation}





% \paragraph{Tradeoff between cache size and lookahead value.}
% There is an inherent tradeoff between lookahead value and cache size. A larger lookahead value will require us to have a large cache size, while  a smaller lookahead value might lead to large amount of churn in the cache. We study how lookahead value effect the cache size, churn and the training throughput in Section~\ref{sec:oracle_cacher_benchmark}. From our analysis we found that a lookahead value of 100 to 200 is optimal and going beyond it leads to diminishing returns(Figure ~\ref{fig:effect_of_lookahead_throughput_oracle_cacher}). 


% When the oracle cacher is processing the 6-th iteration. First, it is launching a prefetch for the embeddings $e$ because there is no request yet to prefetch it. 






\begin{algorithm}[t]
% \scriptsize{}
\small
\caption{Lookahead Algorithm}
\label{alg:lookaheadalg}
\SetKwInOut{KwIn}{Input}
\KwIn{LookAheadValue}

$BatchQueue = Queue()$\;
$LatestTracker = Dictionary()$\;
$InCache = Set()$\;

\While{$\mli{BatchQueue}.size() > 0$} {
 \While{$hasNextBatch()$ and $BatchQueue.size() < LookAheadValue$}{
         $Batch = getNextBatch()$\;
        $IterationNumber = Batch.IterationNum$\;
        \For{\texttt{$\mli{EmbID} \in  Batch.UniqueEmbeddings()$}}{
            $LatestTracker [\mli{EmbID}] = IterationNumber$ \;
            $BatchQueue.pushBack(Batch)$\;
        }
        
        
 }
 $\mli{TTLUpdateRequests} = \{\}$\;
        $CacheFetchRequests = \{\}$\;
        $CurrentBatch =BatchQueue.popFront()$\;
        \For{\texttt{$\mli{EmbID} \in  CurrentBatch.UniqueEmbeddings()$}}{
            $\mli{TTL} = LatestTracker [\mli{EmbID}]$\;
            $\mli{TTLUpdateRequests}.append((\mli{EmbID}, \mli{TTL}))$\;
                    \If {$\mli{EmbID}$ \textnormal{is not in} $InCache$} {

                $CacheFetchRequests.append(\mli{EmbID})$\;
                $InCache.insert(\mli{EmbID})$\;
        }
        \If {$\mli{TTL} = CurrentBatch.number$} {
                $InCache.erase(\mli{EmbID})$\;
                $LatestTracker.erase(\mli{EmbID})$\;
        
        }

        }
                $SendToTrainers(\mli{TTLUpdateRequests})$\;
        $SendToTrainers(CacheFetchRequests)$\;
}
\end{algorithm}
% \vspace{-20pt}
% First we discuss the existing training setup used for Recommendation Model Training. Figure~\ref{fig:existing_training_setup} shows an overview of distributed training setup based on implementation by Facebook~\cite{dlrmopensource}. In a typical DLRM training, neural network(NN) parameters are stored on the GPUs and replicated. The dense NN parameters are trained in data-parallel fashion and   gradients are synchronised using the all-reduce communication collective. However, embedding tables are extremely large to hold in the GPU memory and often can not even fit into the main memory of the system. Therefore, embedding tables are typically partitioned across nodes and stored in main memory and trained in a model-parallel fashion. The embeddings are fetched using all-to-all collective. Figure~\ref{fig:all2all} illustrates the operation of all-to-all collective . Figure~\ref{fig:dlrm_dependency_graph}(left) shows the dependency graph of a DLRM model. In Figure~\ref{fig:dlrm_dependency_graph} (left) we can see how the model allows the possibilty of overlapping several communication heavy steps with compute heavy steps for higher efficiency, \eg the embedding all-to-all fetch can be overlapped with forward pass of bottom NN and similarly gradient synchronization can be overlapped with the backward pass. However, when training with 8 \emph{p3.2xlarge} despite these optimizations we see that only 8.5\% of observed forward and backward pass are spent on compute, rest of the time is spent on embedding fetch and model synchronization. 

% Another observation we have is that existing training setup is very centralized and tied to properties of number of trainers, \ie, we can not scale number of partitions of embedding without increasing number of trainers . We believe this dis-aggregation is extremely important for better resource utilization and scalability. An example of where dis-aggregation of trainers and embedding servers will be useful is when embedding tables are extremely large but the dense neural network parameters are quite small and do not require significant amount of compute. In the existing setup despite not needing additional GPU machines we will have to use them, leading to wastage of resources. Further, the existing training setup completely ignores the skewness in data access pattern of embeddings and will even fetch the same embedding multiple time even when the embedding is repeated within a batch.

% The skewness in access pattern as shown in Figure~\ref{fig:access_cdf} indicates that recommendation model training can benefit significantly from some sort of caching of hot embeddings. However, naive caching a particular set of hot embedding is not enough, primarily because as batch size increases a large number of embeddings are still required to fetched from outside the cache still increasing the training latency significantly. Figure~\ref{fig:hit_rate_batch} shows the distribution of embeddings fetched from the cache as we increase the batch size. Most notably, we see that as batch size increases the ratio of embeddings fetched from the cache to the total number of unique embeddings drastically keeps decreasing, \eg for a batch size of  16,384 only 0.1\% of the total unique embeddings required  are fetched from the cache. This clearly shows that a simple naive caching algorithm will not work. Prior work proposes Frequently Accessed Framework(FAE)~\cite{adnan2021high} which shows that one can pre-process the training data into two different buckets, namely hot examples and cold examples. Examples which access all their embeddings from the cache are considered as hot examples and rest are considered cold. In their system, the authors of FAE~\cite{adnan2021high} then pre-process and segregate the examples comprised completely of hot embeddings. During training for some duration they train using hot batches and during other intervals training is performed on cold batches. However, their system has two drawbacks, firstly it impacts the statistical efficiency training continuously with hot batches and then continuously with cold batches effect the data processing order which has been shown to extensively impact statistical efficiency of training~\cite{}. To mitigate this effect they need to frequently switch between hot and cold embeddings which requires to synchronize caches with the embedding tables stored in memory. Second issue with  FAE~\cite{adnan2021high} is that before training, the data needs to processed into hot or cold examples, even for the relatively small Kaggle Criteo dataset this takes around 20minutes. 


% Apart from the insight of high skewness in embedding access \system relies on one other key insight, \emph{in offline batch training the batches and their contents our predictable}, \ie we can look beyond current batch and exactly find out which embeddings will be accessed by future batches. This insight enables \system to look-ahead beyond the current batch and create a perfect cache. \system uses a dynamic local cache which holds embeddings that will be needed in next several batches.

% The second insight which enables \system in completely removing embedding access and write backs from critical path is that embeddings which are not in the cache will not be updated, this allows \system to launch prefetch of embeddings way before. This makes sure that when a training sample is executed all the embeddings (cold and hot) are available locally. 
% In next section we detail the abstractions introduced by \system and the system design.  
    
\subsection{System Design}
\label{sec:system_design}
% and discussed in Section~\ref{sec:existing_method} 
We next present the end-to-end design of \system{} and discuss how our replicated, dynamic cache is integrated with the training system.
%As shown in , the 
% based on the implementation by Facebook
Existing system designs for distributed training of recommendation models~\cite{dlrmopensource} couple storage and compute resources (Figure~\ref{fig:existing_training_setup}), \ie, we cannot scale the number of embedding table partitions without increasing the number of trainers. We believe \emph{disaggregation} is important for better resource utilization, scalability~\cite{dageville2016snowflake, armbrust2021lakehouse} and fault tolerance. For example, when embedding tables are extremely large but the dense neural network parameters are small and do not require large amounts of compute, an optimal configuration would be to use more servers for embedding tables but have fewer trainers. Thus, we design a disaggregated architecture (Figure~\ref{fig:bagpipe_training_setup}) with four major components: (i) Data Processors (ii) Oracle Cacher (iii) Distributed Trainer (iv) Embedding Servers.

%shows a schematic of our system design.


% which can independently scale different components of training using


 \begin{figure*}[t]
    \includegraphics[width=0.8\linewidth]{images/forward_pass_schematic_no_white.pdf}
    \centering
    \vspace{-0.1in}
    \caption{\small{\textbf{A schematic of how overlapping various operations work}: The above figure shows an illustration of how \system manages to minimize the communication and cache management on the critical path. We show that how \system only synchronizes those embeddings  on the critical path which are going to be used by the next iteration. For example - In iteration we only synchronize embeddings needed in iteration 2 ($E_{iter_2}$). Rest of the embeddings ($E\notin E_{iter_2}$) are synchronized off the critical path. Further before each synchronization of embeddings we have a \emph{Synchronization Point} where we check all off-the-critical synchronization have finished before launching other communications.
    }}
    \label{fig:overlap_schematic}
    \vspace{-15pt}
    \end{figure*}
    

% extremely

% An example of where disaggregation of trainers and embedding servers will be useful is

% To enable dynamic caching and 

%All the components communicate with each other over RPC (we use a mix of asynchronous and synchronous RPCs).
%For our all our other control flow logic  Remote Procedure Calls (RPCs).

%For synchronizing the dense parameters and updates in the dynamic local cache we use the MPI AllReduce primitive.  We next provide details of each of our system component. 

\noindent\textbf{Data Processor.} Data processors are responsible for reading training data and creating batches. Prior work~\cite{zhao2021understanding, mudigere2021software} has shown that data processing for recommendation models is very compute intensive and 
% Data processing if performed on the same node on which training is performed, 
can reduce the throughput of recommendation model training by as much as 56\%~\cite{zhao2021understanding}. Inspired by the design proposed in~\cite{zhao2021understanding} we offload the data processing from the training nodes to remote nodes which are exclusively used for data processing. Depending on throughput requirements the users can scale-up or scale-down the nodes used for data processing. 
%Since the communication is over RPC, the users of \system can also choose to pack data pre-processors with other functionalities as well.

\noindent\textbf{\orc.} %\orc is one of the main components of \system.
%\orc implements the look-ahead routine discussed in Algorithm~\ref{alg:lookaheadalg}. 
\orc is a centralized service which inspects all the processed training batches and determines the cache contents. Using the lookahead algorithm (Algorithm~\ref{alg:lookaheadalg}), \orc decides which elements to prefetch for the current batch and the TTL for eviction of elements being cached.
% which elements to cache from the current batch and
% if the lease (TTL) of an element existing in the cache needs to be updated. 
%\orc is also responsible for routing batches of training data to the workers. 
\orc sends the prefetch requests, training data as well as the cache information using async RPC calls to the trainers.
An important point to note is that the cache changes for an iteration do not happen when the oracle cacher generates the requests. Those requests are sent to the trainers with the iteration number to apply them at. The requests are then applied by the trainer at an appropriate time so as to maintain consistency. 
%To reiterate, state changes to caches is performed by the trainers, the \orc just generates what the trainers are supposed to do and at what iteration. 
%Using the iteration number to coordinate when updates are performed minimizes coordination while providing consistency guarantees.

%This transfer of control to trainers and using the iteration number for coordinating when to perform an action  minimizes the co-ordination required between 
%\orc and training nodes, while providing consistency guarantees. 
 
% partitioning



%  This formulation of \orc provides a subtle but an extremely important guarantee and allows us scale despite providing the same guarantees as synchronous training. When \orc is looking at a batch number $x$, either the  embedding needed by the batch with its most updated value will be available in the cache when the batch is processed or no preceding batch in the lookahead range (any batch number $x - \text{lookahead value}$)   is going to update that specific embedding. To emphasize this again but in a slightly different manner, if an embedding was needed by a batch in batch number range [x-lookahead value, x) it will be in the cache, if it is not in the cache it means no batch in range of $[x-\text{lookahead value}, x)$ is updating it. Therefore as long as the prefetch request is dispatched by the trainer after processing batch number: $x - \text{lookahead value}$, we can safely prefetch those without being concerned about staleness value. This specific condition guarantees that despite fetching embeddings out of order we will still see the same results as synchronous training. This is very similar to out-of-order execution performed in computer-architecture. 
 
 \noindent\textbf{Trainer.} Trainers are GPU machines, which hold the dense neural network portion of recommendation model in the GPU memory. Trainers also hold the dynamic cache in GPU memory where the embeddings needed by future batches are stored. The trainers perform forward and backward passes in a synchronous fashion, \ie at the end of each batch the gradients of the dense neural networks are synchronized. Trainers also perform two other critical operations: (i) prefetching the embeddings based on requests sent by \orc (ii) cache maintenance. The trainers perform prefetching by sending asynchronous requests to \embs.
%  only send prefetching request for a batch if it is within the lookahead value of the most recently processed batch, \ie if $y$ is the most recently processed batch then we will on \shivaram{Maybe say the order in which requests are sent or how many are kept outstanding?} 
Cache maintenance includes addition and eviction of embeddings and updates to the TTL values. To maintain consistency trainers follow the invariant discussed in Section~\ref{sec:caching_in_bagpipe}.

% The trainers ensure consistency by following the invariant of prefetching $x$ only $x - \text{\lkval}$ has been written back (Section~\ref{sec:caching_in_bagpipe}).
 
 %\saurabh{Discuss, we are sort of repeating portions}
 %As discussed previously (Section~\ref{sec:lookahead_routine}), our lookahead provides consistency as long as prefetch requests for embeddings needed by a batch $x$ are dispatched, only after the training and updates for batch $x - \text{\lkval}$  have been propagated to the embedding servers, \eg if \lkval is 40 and $x$ is 100 then as long as prefetch request for remote embeddings (embeddings not in local cache) needed by batch number 100 ($x$) are made after processing batch number 60 ($x - \text{\lkval}$) our formulation will provide consistency guarantees similar to synchronous training.
% For cache evictions all elements whose TTL value is less than currently processed iteration number are evicted. 
 
 
%  (Move in overlap section) All updates to the cache and prefetching are performed in a separate thread thus not affect the training process.  When an embedding is evicted from the cache, the trainer updates the latest value on the \embs by making a synchronous RPC call. We would like to point out that our caching data structure can operate completely lock free, this is because of our lookahead formulation in \orc, it is guaranteed that the training thread and cache maintenance thread will operate on completely different indices of the dynamic cache.
 
 % eviction, addition and update

\noindent\textbf{\embs.} Embedding servers store all the embedding tables and act as a sharded parameter server. They handle the prefetch and update requests from the trainer. Typically an \embs runs on a high memory machine due to the large size of embedding tables. 
%We use the Embedding Bag abstraction~\cite{embbag} provided by PyTorch to store the embeddings. 
The \embs exposes two RPC functions, one to fetch embeddings and the other to receive updated embeddings from the trainers.
%and correspondingly update the local version based on the new values.  % and send to trainers

\subsection{Overlapping communication with compute}
\label{sec:bagpipe_overlap}
% cache management and
% \shivaram{move this before fault tolerance}
\system is designed to minimize any additional compute and communication on the critical path of training. To achieve this we use the idea of overlapping all such operations with computation of forward and backward pass that take place on the trainers. Figure~\ref{fig:overlap_schematic} shows a schematic of how \system can potentially hide most of the extra overhead by overlapping the prefetch and cache maintenance actions described before with the compute required for model training. We next describe optimizations we design to achieve this.




% We next detail how we utilize our formulation to remove almost all communication and additional compute out of the critical path.

\paragraph{Overlapping cache management with training.} Cache management in \system consists of primarily three operations. First, we need to update the TTL of elements in the cache based on values sent by \orc. Second, we need to evict the elements which have TTL less than current iteration number and upon eviction we need to update the latest value on the \embs by making a RPC call. Third, we need to launch prefetch requests sent by \orc, for any iteration number which is needed within next \lkval batches, \ie if the current iteration number is $x$ we should launch prefetch requests for an iteration number $(x, x+\text{\lkval}]$. 

We perform, all cache management operations in a separate thread thus not affecting the training process. We would like to point out that our caching data structure can operate completely lock free, because in our lookahead formulation in \orc, it is guaranteed that the training thread and cache maintenance thread will operate on completely separate indices of the dynamic cache.  This guarantee stems from how we prefetch and evict, \eg, Assuming we are currently training batch $x$ and lookahead value $L$, for a batch in range [x+1, x+L], we will only be prefetching an embedding which is not being used by training batch $x$. At the same time we only evict an embedding which will not be used by any batch in range [x, x+L]. This ensures that none of the embeddings that are being accessed by the cache management thread will be accessed by the training thread during batch $x$, thus requiring no locks.
The training thread sends a signal to the cache management thread indicating which iteration number has finished and no other additional synchronization is required.  
This ensures that cache management has minimal overhead.

% the cache management thread 
%formulation
% setup
% only
% main 
%   different portions of the cache than the training thread

\paragraph{Overlapping Cache Synchronization.} Replicated Caches need to be synchronized and this synchronization happens after the forward/backward compute, on the critical path of training. We perform two additional optimizations to improve the performance of synchronization. First, instead of synchronizing the whole cache we only synchronize gradients of the elements which have been updated in the current iteration. Further, we only synchronize the elements which will be required in the next iteration on the critical path. We schedule rest of the elements to be synchronized in the background. Thus, only a very small portion of the cache entries are synchronized on the critical path. From our experiments on Kaggle Criteo dataset with 8 \emph{p3.2xlarge} and batch size of 16,384, on a single machine, these optimizations lead to an average 3,471 entries out of 14,184 entries that need to be synchronized on critical path.
%leads to an update vector on avg of 14,184 elements out of which only on a. 
Thus, our optimizations reduce the communication on critical path by almost 75\%, and help us overlap a large portion of cache synchronization with compute. We evaluate the effect of these optimizations in Section~\ref{sec:oracle_cacher_benchmark}

% separately
% we perform an additional optimization in which 

\subsection{Fault Tolerance} 
\label{sec:ft}
The frequency of job failures in ML training clusters~\cite{gupta2017failures,jeon2019analysis} and the opportunity to use pre-emptible machines in the cloud (e.g., spot instances) to reduce costs, makes fault tolerance an important concern. 
However, given the extremely large model sizes, enabling fault tolerance for recommendation models through regular check-pointing is challenging. Checkpointing large models can take several minutes~\cite{eisenman2022check} during which the compute resources stay idle. 
% large
%However, 
%cloud environment where data scientists frequently use   to train models in order
%extremely important as failure rates are pretty high. 
Recent work~\cite{eisenman2022check} has proposed mechanisms for checkpointing recommendation models for the DLRM design discussed in Section~\ref{sec:existing_method} and other prior methods~\cite{maeng2021understanding} only checkpoint frequently updated embeddings, thus sacrificing consistency.
We next discuss how our disaggregated design in \system can enable low overhead fault tolerance without compromising on consistency.
%We next discuss the fault tolerance of each individual component of \system. 

% of training
% instead of all the updated embeddings

% \shivaram{why does prior work sacrifice consistency. Not clear}\saurabh{added a sentence check}

\noindent\textbf{\orc.} \orc is designed such that all the necessary internal state is also present on the trainers. Therefore, whenever \orc has to be restarted we only need to fetch the last iteration number processed by the trainers and the embedding IDs present on them. Even if one trainer is available, \orc can be restarted using its state.

\noindent\textbf{Trainers.} Since the trainers proceed in a lock step fashion and maintain a replicated cache, as long as even one trainer is available \system can recover from a trainer failures. When \orc observes that a trainer has failed, it first requests the cloud service provider for additional training machines to compensate for the lost trainers. While the machine is being allocated, \orc makes an RPC call to ask an existing trainer to checkpoint its state (model parameters and cache contents) and then copies this state to the newly allocated trainer. We evaluate the overhead of this in Section~\ref{sec:eval}.

\noindent\textbf{Embedding Server.} Embedding Servers hold the embedding tables which are often extremely large. Our design doesn't make any changes to embedding servers when compared to prior DLRM designs~\cite{eisenman2022check} and thus we can use the same techniques as suggested in Check-n-Run~\cite{eisenman2022check} to checkpoint embedding servers periodically.



%Embedding server can be continuously checkpointed using a similar scheme as used by InnoDB to create backups of running database. At the beginning of checkpointing we instantiate a write buffer which holds the write updates, while the embedding tables are made read only to provide consistent checkpointed. During checkpointing all the updates are written to the write buffer. While for reads we first check if the embedding is available in write buffer if not present in the write buffer we read the embedding from the read only embedding table. This guarantees that the checkpoint is consistent and training proceeds while the checkpoint is being taken.
%In subsequent future work we will provide more details on how our design enables fault tolerance with almost no overhead. 






==> discussion.tex <==
% \vspace{-5pt}

% In our current design \orc is not horizontally scalable. H

% owever, the overhead of \orc is extremely small even for extremely large batch sizes and lookahead values. In \S\ref{sec:oracle_cacher_benchmark} we find that \orc, even for large batch size of 131K, can dispatch 3.27 Million samples per second. This is sufficient to power the most optimized large scale systems reported in prior work, \eg 8 ZionEx nodes (128 A100 GPUs) which process up to 1.6 Million samples per second~\cite{mudigere2021software}.
%.  we study the scalability of \orc.


